RAFT-MSF: Self-Supervised Monocular Scene Flow using Recurrent Optimizer

Learning scene flow from a monocular camera still remains a challenging task due to its ill-posedness as well as lack of annotated data. Self-supervised methods demonstrate learning scene flow estimation from unlabeled data, yet their accuracy lags behind (semi-)supervised methods. In this paper, we introduce a self-supervised monocular scene flow method that substantially improves the accuracy over the previous approaches. Based on RAFT, a state-of-the-art optical flow model, we design a new decoder to iteratively update 3D motion fields and disparity maps simultaneously. Furthermore, we propose an enhanced upsampling layer and a disparity initialization technique, which overall further improves accuracy up to 7.2%. Our method achieves state-of-the-art accuracy among all self-supervised monocular scene flow methods, improving accuracy by 34.2%. Our fine-tuned model outperforms the best previous semi-supervised method with 228 times faster runtime. Code will be publicly available.

==> figures/main_fig.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\begin{figure*}
\centering
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Image [id:dp18665258292755182] 
\draw (80.5,135) node  {\includegraphics[width=74.25pt,height=22.5pt]{figures/000014_10.png}};
%Image [id:dp17350722949856645] 
\draw (80.5,74.99) node  {\includegraphics[width=74.25pt,height=22.48pt]{figures/000014_11.png}};
%Image [id:dp5340399321382765] 
\draw (80.5,194.99) node  {\includegraphics[width=74.25pt,height=22.48pt]{figures/000014_10.png}};
%Rounded Rect [id:dp38507203373168863] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=0.75]  (157,68) .. controls (157,63.58) and (160.58,60) .. (165,60) -- (244,60) .. controls (248.42,60) and (252,63.58) .. (252,68) -- (252,92) .. controls (252,96.42) and (248.42,100) .. (244,100) -- (165,100) .. controls (160.58,100) and (157,96.42) .. (157,92) -- cycle ;
%Rounded Rect [id:dp5479132123964887] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (157,128) .. controls (157,123.58) and (160.58,120) .. (165,120) -- (244,120) .. controls (248.42,120) and (252,123.58) .. (252,128) -- (252,152) .. controls (252,156.42) and (248.42,160) .. (244,160) -- (165,160) .. controls (160.58,160) and (157,156.42) .. (157,152) -- cycle ;
%Rounded Rect [id:dp3158944915156183] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.84 ] (160,188) .. controls (160,183.58) and (163.58,180) .. (168,180) -- (247,180) .. controls (251.42,180) and (255,183.58) .. (255,188) -- (255,212) .. controls (255,216.42) and (251.42,220) .. (247,220) -- (168,220) .. controls (163.58,220) and (160,216.42) .. (160,212) -- cycle ;
%Straight Lines [id:da5281986394528402] 
\draw    (130,80) -- (155,80) ;
\draw [shift={(157,80)}, rotate = 179] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da5324761943150698] 
\draw    (130,140) -- (155,140) ;
\draw [shift={(158.14,140)}, rotate = 178.84] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da903712814622923] 
\draw    (130,200) -- (155,200) ;
\draw [shift={(160.71,200)}, rotate = 179.47] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Shape: Cube [id:dp21235581306658813] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.41 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=0.75]  (281.01,49.3) -- (287.3,42.99) -- (302,42.96) -- (302.1,96.66) -- (295.82,102.97) -- (281.12,103) -- cycle ; \draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.41 ][line width=0.75]  (302,42.96) -- (295.71,49.27) -- (281.01,49.3) ; \draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.41 ][line width=0.75]  (295.71,49.27) -- (295.82,102.97) ;
%Shape: Cube [id:dp20873374199693862] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.41 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=0.75]  (281.01,115.3) -- (287.3,108.99) -- (302,108.96) -- (302.1,162.66) -- (295.82,168.97) -- (281.12,169) -- cycle ; \draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.41 ][line width=0.75]  (302,108.96) -- (295.71,115.27) -- (281.01,115.3) ; \draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.41 ][line width=0.75]  (295.71,115.27) -- (295.82,168.97) ;
%Shape: Cube [id:dp40540417807098983] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.41 ][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=0.84 ][line width=0.75]  (281.01,181.3) -- (287.3,174.99) -- (302,174.96) -- (302.1,228.66) -- (295.82,234.97) -- (281.12,235) -- cycle ; \draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.41 ][line width=0.75]  (302,174.96) -- (295.71,181.27) -- (281.01,181.3) ; \draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.41 ][line width=0.75]  (295.71,181.27) -- (295.82,234.97) ;
%Rounded Rect [id:dp5719920046117468] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.84 ][fill={rgb, 255:red, 208; green, 33; blue, 2 }  ,fill opacity=1 ] (341.86,68) .. controls (341.86,63.58) and (345.44,60) .. (349.86,60) -- (403.86,60) .. controls (408.28,60) and (411.86,63.58) .. (411.86,68) -- (411.86,92) .. controls (411.86,96.42) and (408.28,100) .. (403.86,100) -- (349.86,100) .. controls (345.44,100) and (341.86,96.42) .. (341.86,92) -- cycle ;
%Straight Lines [id:da9984199172711905] 
\draw    (251,78) -- (277.02,78) ;
\draw [shift={(280,78)}, rotate = 181.39] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da9132548102232989] 
\draw    (251,140) -- (277,140) ;
\draw [shift={(280,140)}, rotate = 180.7] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da29756976178622296] 
\draw    (255,200) -- (277,200) -- (278.29,201.18) ;
\draw [shift={(280,200)}, rotate = 180.93] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da3173351480533453] 
\draw    (302.43,77.29) -- (339.45,77.94) ;
\draw [shift={(342.45,77.99)}, rotate = 181.01] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Rounded Rect [id:dp07744949227501619] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.84 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.84 ] (344,127.86) .. controls (344,123.44) and (347.58,119.86) .. (352,119.86) -- (419.29,119.86) .. controls (423.7,119.86) and (427.29,123.44) .. (427.29,127.86) -- (427.29,151.86) .. controls (427.29,156.28) and (423.7,159.86) .. (419.29,159.86) -- (352,159.86) .. controls (347.58,159.86) and (344,156.28) .. (344,151.86) -- cycle ;
%Straight Lines [id:da07954835536512705] 
\draw    (303,140.29) -- (341.02,140.94) ;
\draw [shift={(344.02,140.99)}, rotate = 180.98] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da0516391145288666] 
\draw    (320.89,77.63) -- (321,131.29) ;
%Straight Lines [id:da372997025910061] 
\draw    (321,131.29) -- (340.86,131.78) ;
\draw [shift={(343.86,131.86)}, rotate = 181.43] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Rounded Rect [id:dp31918540996959455] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.84 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.69 ] (468.6,124.6) .. controls (468.6,120.18) and (472.18,116.6) .. (476.6,116.6) -- (540.6,116.6) .. controls (545.02,116.6) and (548.6,120.18) .. (548.6,124.6) -- (548.6,148.6) .. controls (548.6,153.02) and (545.02,156.6) .. (540.6,156.6) -- (476.6,156.6) .. controls (472.18,156.6) and (468.6,153.02) .. (468.6,148.6) -- cycle ;
%Straight Lines [id:da1787123507468269] 
\draw    (428.29,140) -- (466.3,140.65) ;
\draw [shift={(469.3,140.7)}, rotate = 180.98] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Image [id:dp6948156277490034] 
\draw (618.7,164) node  {\includegraphics[width=74.25pt,height=22.5pt]{figures/14_disp.jpg}};
%Image [id:dp719939307141809] 
\draw (617.5,108.6) node  {\includegraphics[width=74.25pt,height=22.5pt]{figures/14_resize_sf.png}};
%Straight Lines [id:da33083712210568295] 
\draw    (548.6,138.2) -- (565.73,111.8) ;
\draw [shift={(567.37,109.29)}, rotate = 122.99] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da5341645733406297] 
\draw    (548.6,138.2) -- (566.43,166.42) ;
\draw [shift={(568.03,168.95)}, rotate = 237.71] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da2366584006821093] 
\draw    (302.53,200.53) -- (501.98,199.94) ;
%Straight Lines [id:da4450294030710831] 
\draw    (501.98,199.94) -- (501.79,160.72) ;
\draw [shift={(501.78,157.72)}, rotate = 89.73] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da5505125641386786] 
\draw    (411.57,78.37) -- (501.22,77.97) ;
%Straight Lines [id:da2581401642674015] 
\draw    (501.22,77.97) -- (502.12,114) ;
\draw [shift={(502.2,117)}, rotate = 268.56] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;

% Text Node
\draw (45,48) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Source frame }};
% Text Node
\draw (45,107) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Target frame}};
% Text Node
\draw (45,168) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small Source frame }};
% Text Node
\draw (163,73) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Feature Network}};
% Text Node
\draw (163,133) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Feature Network}};
% Text Node
\draw (163,193) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Feature Network}};
% Text Node
\draw (352,72) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Depth init}};
% Text Node
\draw (352,132) node [anchor=north west][inner sep=0.75pt]   [align=left] {Corellation};
% Text Node
\draw (487,131) node [anchor=north west][inner sep=0.75pt]   [align=left] {Update};


\end{tikzpicture}
\caption{\textbf{Overview of our method}. Feature networks encode input images to feature vectors. Correlation volume is constructed by using encoded features. We initialize 3D motion field to zeros everywhere and disparity is initialized using 2 convolutional layers as in Depth Int. During each iteration, the update operator uses the current estimates of scene flow and disparity to index from the correlation pyramid. The output of the update operator is fed to scene flow and disparity heads. The scene flow can be projected to optical flow.}
\label{fig:main_fig}
\end{figure*}

==> figures/update_fig.tex <==
\begin{figure}[t]
\centering

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,483); %set diagram left start at 0, and has height of 483

%Straight Lines [id:da0315194845950828] 
\draw    (107,132.99) -- (128.89,132.66) ;
\draw [shift={(131.89,132.61)}, rotate = 179.12] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da5630346090176328] 
\draw    (107,162) -- (127.57,161.78) ;
\draw [shift={(130.57,161.75)}, rotate = 179.38] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da22585194747228576] 
\draw    (107,175) -- (128.97,175.28) ;
\draw [shift={(131.97,175.32)}, rotate = 180.75] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da7985249254992222] 
\draw    (107,148) -- (127.1,147.86) ;
\draw [shift={(130.1,147.84)}, rotate = 179.6] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Rounded Rect [id:dp8093153862046798] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.84 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.84 ] (130,138.01) .. controls (130,132.49) and (134.48,128.01) .. (140,128.01) -- (200,128.01) .. controls (205.52,128.01) and (210,132.49) .. (210,138.01) -- (210,168.01) .. controls (210,173.54) and (205.52,178.01) .. (200,178.01) -- (140,178.01) .. controls (134.48,178.01) and (130,173.54) .. (130,168.01) -- cycle ;
%Straight Lines [id:da6234928769921382] 
\draw    (266.58,154.06) -- (280.23,153.66) ;
\draw [shift={(283.22,153.57)}, rotate = 178.32] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Shape: Cube [id:dp1778420391716451] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=0.84 ][fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.84 ] (223.53,142.26) -- (232.15,133.65) -- (236.89,133.65) -- (236.89,161.77) -- (228.27,170.39) -- (223.53,170.39) -- cycle ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=0.84 ] (236.89,133.65) -- (228.27,142.26) -- (223.53,142.26) ; \draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=0.84 ] (228.27,142.26) -- (228.27,170.39) ;
%Straight Lines [id:da22124263182922466] 
\draw    (237.6,153.21) -- (254.58,153.08) ;
\draw [shift={(257.58,153.06)}, rotate = 179.55] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Flowchart: Summing Junction [id:dp955722010674259] 
\draw   (256.58,154.06) .. controls (256.58,151.3) and (258.82,149.06) .. (261.58,149.06) .. controls (264.34,149.06) and (266.58,151.3) .. (266.58,154.06) .. controls (266.58,156.82) and (264.34,159.06) .. (261.58,159.06) .. controls (258.82,159.06) and (256.58,156.82) .. (256.58,154.06) -- cycle ; \draw   (258.04,150.52) -- (265.11,157.59) ; \draw   (265.11,150.52) -- (258.04,157.59) ;
%Straight Lines [id:da5001794383010534] 
\draw    (109.8,190.08) -- (259.86,190.31) ;
%Straight Lines [id:da6745032247932414] 
\draw    (259.86,190.31) -- (260.16,161.65) ;
\draw [shift={(260.19,158.65)}, rotate = 90.6] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Rounded Rect [id:dp4672733812125105] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.84 ][fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.83 ] (283.39,143.67) .. controls (283.39,140.35) and (286.07,137.67) .. (289.39,137.67) -- (337.39,137.67) .. controls (340.7,137.67) and (343.39,140.35) .. (343.39,143.67) -- (343.39,161.67) .. controls (343.39,164.98) and (340.7,167.67) .. (337.39,167.67) -- (289.39,167.67) .. controls (286.07,167.67) and (283.39,164.98) .. (283.39,161.67) -- cycle ;
%Straight Lines [id:da4066254147112154] 
\draw    (209.98,153.66) -- (220.66,153.63) ;
\draw [shift={(223.66,153.62)}, rotate = 179.86] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (5.36,-2.57) -- (0,0) -- (5.36,2.57) -- cycle    ;
%Straight Lines [id:da22934536515307746] 
\draw    (344.01,153.25) -- (350.95,153.1) ;
%Straight Lines [id:da43402553931528276] 
\draw    (350.95,153.1) -- (361.23,142.83) ;
\draw [shift={(363.35,140.7)}, rotate = 135] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (3.57,-1.72) -- (0,0) -- (3.57,1.72) -- cycle    ;
%Rounded Rect [id:dp5199668214435151] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.84 ][fill={rgb, 255:red, 139; green, 87; blue, 42 }  ,fill opacity=0.85 ] (353,124.26) .. controls (353,122.05) and (354.79,120.26) .. (357,120.26) -- (400.2,120.26) .. controls (402.41,120.26) and (404.2,122.05) .. (404.2,124.26) -- (404.2,136.26) .. controls (404.2,138.47) and (402.41,140.26) .. (400.2,140.26) -- (357,140.26) .. controls (354.79,140.26) and (353,138.47) .. (353,136.26) -- cycle ;
%Straight Lines [id:da6762973718778469] 
\draw    (350.95,153.1) -- (362.62,153.38) ;
\draw [shift={(365.62,153.45)}, rotate = 181.36] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (3.57,-1.72) -- (0,0) -- (3.57,1.72) -- cycle    ;
%Rounded Rect [id:dp09567556719489434] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.84 ][fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.84 ] (365.94,148.72) .. controls (365.94,146.52) and (367.73,144.72) .. (369.94,144.72) -- (411.4,144.72) .. controls (413.61,144.72) and (415.4,146.52) .. (415.4,148.72) -- (415.4,160.72) .. controls (415.4,162.93) and (413.61,164.72) .. (411.4,164.72) -- (369.94,164.72) .. controls (367.73,164.72) and (365.94,162.93) .. (365.94,160.72) -- cycle ;
%Straight Lines [id:da4179003592591244] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (350.95,153.1) -- (363.58,167.91) (360.48,158.12) -- (354.39,163.31) ;
\draw [shift={(365.52,170.19)}, rotate = 229.53] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (3.57,-1.72) -- (0,0) -- (3.57,1.72) -- cycle    ;
%Rounded Rect [id:dp057290511078173845] 
\draw  [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=0.84 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.84 ] (353,174.77) .. controls (353,172.56) and (354.79,170.77) .. (357,170.77) -- (395.8,170.77) .. controls (398.01,170.77) and (399.8,172.56) .. (399.8,174.77) -- (399.8,186.77) .. controls (399.8,188.98) and (398.01,190.77) .. (395.8,190.77) -- (357,190.77) .. controls (354.79,190.77) and (353,188.98) .. (353,186.77) -- cycle ;
%Shape: Rectangle [id:dp4139527166910659] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][dash pattern={on 1.69pt off 2.76pt}][line width=1.5]  (102.67,118.71) -- (420.6,118.71) -- (420.6,194.42) -- (102.67,194.42) -- cycle ;

% Text Node
\draw (105,133) node [anchor=north west][inner sep=4.5pt]   [align=left] {{\small $s_{k}$}};
% Text Node
\draw (105,115) node [anchor=north west][inner sep=4.5pt]   [align=left] {{\small $d_{k}$}};
% Text Node
\draw (102.5,158) node [anchor=north west][inner sep=4.5pt]   [align=left] {{\small $L_{C}$}};
% Text Node
\draw (107.5,181) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small $c_{\theta}$}};
% Text Node
\draw (107.5,149) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small $F$}};
% Text Node
\draw (138,147) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small MF Encoder}};
% Text Node
\draw (300,147) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small GRU}};
% Text Node
\draw (260,112) node   [align=left] {\begin{minipage}[lt]{68pt}\setlength\topsep{0pt}
{\small Update Operator}
\end{minipage}};
% Text Node
\draw (353.5,124) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small disp head}};
% Text Node
\draw (372,148) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small sf head}};
% Text Node
\draw (363,174) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\small mask}};
% Text Node
\draw (270,128) node   [align=left] {\begin{minipage}[lt]{68pt}\setlength\topsep{0pt}
{\small MF}
\end{minipage}};


\end{tikzpicture}

\caption{\textbf{A detailed view of the update operator}: Motion Feature (MF) Encoder encodes current estimates disparity $d_{k}$, scene flow $s_{k}$, 2D Flow $F$, and correlation features $L_{C}$ to motion features, which is concatenated with context features $c_{\theta}$ and passed to GRU. Disp and Sf heads are used to decode disparity and scene flow estimates, and mask head is used produce convex mask for upsampling. }
\label{fig:update_fig}
\end{figure}
